Clustering RDF Databases Using Tunable-LSH

The Resource Description Framework (RDF) is a W3C standard for representing graph-structured data, and SPARQL is the standard query language for RDF. Recent advances in Information Extraction, Linked Data Management and the Semantic Web have led to a rapid increase in both the volume and the variety of RDF data that are publicly available. As businesses start to capitalize on RDF data, RDF data management systems are being exposed to workloads that are far more diverse and dynamic than what they were designed to handle. Consequently, there is a growing need for developing workload-adaptive and self-tuning RDF data management systems. To realize this vision, we introduce a fast and efficient method for dynamically clustering records in an RDF data management system. Specifically, we assume nothing about the workload upfront, but as SPARQL queries are executed, we keep track of records that are co-accessed by the queries in the workload and physically cluster them. To decide dynamically (hence, in constant-time) where a record needs to be placed in the storage system, we develop a new locality-sensitive hashing (LSH) scheme, Tunable-LSH. Using Tunable-LSH, records that are co-accessed across similar sets of queries can be hashed to the same or nearby physical pages in the storage system. What sets Tunable-LSH apart from existing LSH schemes is that it can auto-tune to achieve the aforementioned clustering objective with high accuracy even when the workloads change. Experimental evaluation of Tunable-LSH in our prototype RDF data management system, chameleon-db, as well as in a standalone hashtable shows significant end-to-end improvements over existing solutions.

==> fig/storage-system.tex <==
\begin{tikzpicture}
	\newcommand{\boxWidth}{15cm}
	\newcommand{\boxHeight}{6cm}
	\newcommand{\boxSmallHeight}{2cm}
	\newcommand{\boxExtraSmallHeight}{1cm}
	\newcommand{\boxSmallWidthA}{11cm}
	\newcommand{\boxSmallWidthB}{3cm}
	\newcommand{\textMargin}{1cm}

	\newcommand{\bufferPoolPage}[3]{

		\node (p1) [draw, left of=#1, xshift=#2, yshift=#3, rounded corners=2pt, minimum width=2cm, minimum height=2cm] {};
	
		\node (r11) [draw, left of=p1, xshift=0.5cm, yshift=0.75cm, minimum width=0.8cm, minimum height=0.4cm] {};
		\node (r13) [draw, left of=p1, xshift=1.5cm, yshift=0.75cm, minimum width=0.8cm, minimum height=0.4cm] {};

		\node (r21) [draw, left of=p1, xshift=0.5cm, yshift=0.25cm, minimum width=0.8cm, minimum height=0.4cm] {};
		\node (r23) [draw, left of=p1, xshift=1.5cm, yshift=0.25cm, minimum width=0.8cm, minimum height=0.4cm] {};

		\node (r31) [draw, left of=p1, xshift=0.5cm, yshift=-0.25cm, minimum width=0.8cm, minimum height=0.4cm] {};
		\node (r33) [draw, left of=p1, xshift=1.5cm, yshift=-0.25cm, minimum width=0.8cm, minimum height=0.4cm] {};

		\node (r11) [draw, left of=p1, xshift=0.5cm, yshift=-0.75cm, minimum width=0.8cm, minimum height=0.4cm] {};
		\node (r13) [draw, left of=p1, xshift=1.5cm, yshift=-0.75cm, minimum width=0.8cm, minimum height=0.4cm] {};
	}

	\node (box_buffer_pool) [draw, 
		rounded corners=10pt,
		line width=0.5mm,
		minimum width=\boxWidth, 
		minimum height=\boxHeight, 
		text width={\boxWidth-\textMargin}] 
			{\Large \textbf{Buffer \\ Pool}};

	\node (box_cache) [draw,
		above of=box_buffer_pool,
		xshift={ (\boxSmallWidthA - \boxWidth) / 2 },
		yshift={ \boxHeight - 2.5cm },
		rounded corners=10pt,
		line width=0.5mm,
		minimum width=\boxSmallWidthA, 
		minimum height=\boxSmallHeight, 
		text width={\boxSmallWidthA-\textMargin}] 
			{\Large \textbf{Database \\ Cache}};

	%%% Draw zigzag inside cache...
	\draw[decoration = {zigzag,segment length = 3mm, amplitude = 1mm}, decorate] ($(box_cache) + (1.75,1)$)--($(box_cache) + (1.75,-1)$);

	\node (box_tunable_lsh) [draw,
		above of=box_buffer_pool,
		xshift={ (\boxWidth - \boxSmallWidthB) / 2},
		yshift={ \boxHeight - 2.5cm },
		rounded corners=10pt,
		line width=0.5mm,
		minimum width=\boxSmallWidthB, 
		minimum height=\boxSmallHeight, 
		text width={ \boxSmallWidthB - \textMargin }] 
			{ \Large \textbf{Hash Fn.} };

	\node (box_lookup_table) [draw,
		above of=box_cache,
		xshift={ (\boxWidth - \boxSmallWidthA) / 2 },
		yshift={ \boxExtraSmallHeight },
		rounded corners=10pt,
		line width=0.5mm,
		minimum width=\boxWidth, 
		minimum height=\boxExtraSmallHeight, 
		text width={ \boxWidth - \textMargin }] 
			{\Large \textbf{Lookup \\ Table}};

	%%% Draw pages inside [box_buffer_pool]...
	\bufferPoolPage{box_buffer_pool}{-1.5cm}{1.5cm}	
	\bufferPoolPage{box_buffer_pool}{1cm}{1.5cm}
	\bufferPoolPage{box_buffer_pool}{3.5cm}{1.5cm}
	\bufferPoolPage{box_buffer_pool}{6cm}{1.5cm}

	\bufferPoolPage{box_buffer_pool}{-1.5cm}{-1.55cm}
	\bufferPoolPage{box_buffer_pool}{1cm}{-1.55cm}
	\bufferPoolPage{box_buffer_pool}{3.5cm}{-1.55cm}
	\bufferPoolPage{box_buffer_pool}{6cm}{-1.55cm}

	%%% Draw records inside [box_cache]	
	\node (ra1) [draw, left of=box_cache, xshift=0cm, yshift=0.5cm, minimum width=0.8cm, minimum height=0.4cm] {};
	\node (ra2) [draw, left of=box_cache, xshift=1cm, yshift=0.5cm, minimum width=0.8cm, minimum height=0.4cm] {};
	\node (ra3) [draw, left of=box_cache, xshift=2cm, yshift=0.5cm, minimum width=0.8cm, minimum height=0.4cm] {};
	\draw [decorate,line width=1pt,decoration={brace, mirror, amplitude=10pt}] ($(ra1.south west) + (-0.1cm, -0.1cm)$) -- ($(ra3.south east) + (0.1cm, -0.1cm)$)
			node [black, midway, yshift=-0.7cm] {\large \textbf{Warm}};

	\node (rb1) [draw, left of=box_cache, xshift=3.5cm, yshift=0.5cm, minimum width=0.8cm, minimum height=0.4cm] {};
	\node (rb2) [draw, left of=box_cache, xshift=4.5cm, yshift=0.5cm, minimum width=0.8cm, minimum height=0.4cm] {};
	\node (rb3) [draw, left of=box_cache, xshift=5.5cm, yshift=0.5cm, minimum width=0.8cm, minimum height=0.4cm] {};
	\draw [decorate,line width=1pt,decoration={brace, mirror, amplitude=10pt}] ($(rb1.south west) + (-0.1cm, -0.1cm)$) -- ($(rb3.south east) + (0.1cm, -0.1cm)$)
			node [black, midway, yshift=-0.7cm] {\large \textbf{Non-clusterable}};

	%%% Draw pointers inside [box_lookup_table]
	\node (pointer1) [draw, left of=box_lookup_table, xshift=-2cm, yshift=0.0cm, minimum width=2cm, minimum height=1cm] {\large \textbf{\#A$\mathbf{312}$}};
	\node (pointer1) [draw, left of=box_lookup_table, xshift=0cm, yshift=0.0cm, minimum width=2cm, minimum height=1cm] {\large \textbf{\#B$\mathbf{012}$}};

	\node (pointer1) [draw, left of=box_lookup_table, xshift=2.5cm, yshift=0.0cm, minimum width=1cm, minimum height=0.8cm, color=white, text=black] {\Large $\mathbf{\cdots}$};

	\node (pointer1) [draw, left of=box_lookup_table, xshift=5cm, yshift=0.0cm, minimum width=2cm, minimum height=1cm] {\large \textbf{\#AA$\mathbf{00}$}};	
	\node (pointer1) [draw, left of=box_lookup_table, xshift=7cm, yshift=0.0cm, minimum width=2cm, minimum height=1cm] {\large \textbf{\#$\mathbf{104}$F}};	

	\draw [decorate,line width=1pt,decoration={brace, mirror, amplitude=10pt}] ($(box_buffer_pool.south east) + (-1.25cm, 0.5cm)$) -- ($(box_buffer_pool.north east) + (-1.25cm, -0.5cm)$)
			node [black, midway, rotate=90, yshift=-0.6cm] {\large \textbf{Pages}};
\end{tikzpicture}


==> sections/caching.tex <==
\begin{figure}
	\begin{center}
		\inputTikZ{0.5}{fig/storage-system.tex}
	\end{center}
	\caption{Overview of in-memory storage system}
	\label{fig:memory-storage-system}
\end{figure}

Records in the database can be physically clustered using \tunableLSH as shown in Fig.~\ref{fig:adaptive-record-placement}.
In this paper, we focus on two scenarios.
The first one is an in-memory implementation, in which records are primarily stored in the computer's main memory.\footnote{We are not concerned with durability issues and/or non-volatile storage.}
The main-memory storage system is organized in a two-level hierarchy that consists of
	a small-sized database cache for keeping the ``warm" records, and
	a much larger buffer pool for storing all of the records in the database.
The objective is to physically cluster records in the buffer pool 
	to increase CPU cache utilization 
	so that next time a query is executed,
	records can be retrieved more efficiently.

The outcome of \tunableLSH is not deterministic across consecutive calls to the function.
In other words, the same record can be hashed to different buffer pool pages at different times.
Therefore, one needs to keep track of the current mapping between record identifiers and page numbers,
	which incurs the extra overhead of accessing a lookup table prior to retrieving records from the buffer pool.
Naturally, one would not have this problem in conventional hashing.
Nevertheless, this overhead is often amortized by the fact that
	queries typically access multiple records at once.

Fig.~\ref{fig:memory-storage-system} illustrates a possible configuration of the storage system for 
	a $4$GB buffer pool with
	$512$-byte records ($8$-byte headers for record identifiers \verb!+! $504$-byte content) and
	$64$KB pages.
In this configuration, there are $2^{16}$ pages in total, thus, 
	for each record, one needs to allocate a $2$-byte slot in the lookup table 
	to keep track of current record locations (i.e., page numbers).
This adds up to $16$MB in total.
The size of the database cache is adjustable, and in our experiments, we set it to $64$MB.
The hash function also consumes memory, but its size fluctuates dynamically.
That is, as an optimization,
	unless a record utilization counter contains a digit with a non-zero value,
	space is not allocated for it.
Since \tunableLSH considers only the last $k$ queries, one can expect a majority of
	the record utilization counters to be zero (hence, also the memory overhead of \tunableLSH to be low).
In our experiments, the space consumed by \tunableLSH averages ...

No matter how accurate \tunableLSH might be,
	there will always be cases in which
	a noteworthy number of records that are related to the same query
	are scattered across multiple pages.
For example, according to our experiments, 
	on average, $\%$ of the records related to a query are clustered within a single page, whereas
	the remaining $\%$ are scattered across $\Box$ pages.
This is not desirable because we would like to minimize the total number of pages that are accessed per query.
Therefore, to reduce CPU cache stalls due to ``non-clusterable" records,
	we reserve a portion of the database cache for records that have not been properly clustered by \tunableLSH.

Next, we describe how a sequence of 
	\textsc{Prepare}(uint [] \emph{rec\_array}), \textsc{Next}(), $\ldots$, \textsc{Next}()
	methods are executed by the storage system.
\textsc{Prepare} method takes an array of unsigned integers that correspond to record identifiers and
	is responsible for preparing the system for reading, while
	the subsequent \textsc{Next}() calls actually fetch the records
	(not necessarily in the order supplied in \textsc{Prepare}).
More specifically, the \textsc{Prepare} method generates a set of (distinct)
	buffer page identifiers that need to be visited.
Then, these buffer pages are scanned one by one in subsequent calls to \textsc{Next}(),
	while fetching all the relevant records
	and ignoring the ones that are not matched by any identifier in \emph{rec\_array}.
At the end of the last call to \textsc{Next}, 
	\emph{rec\_array} is passed on to the \textsc{Tune} method in Algorithm~\ref{alg:overview:tune}
	to update \tunableLSH.

In the meantime, the fetched records are sent also to the database cache.
We rely on the admission policy of the database cache to determine which records are ``warm".
After \tunableLSH is updated, it is used for determining if any of these ``warm" records involved
	in the \textsc{Prepare} method need to be relocated.
If a record is relocated, the lookup table must also be updated.

Note that if properly configured, nothing prevents \tunableLSH from being used in a disk-based system.
That is, relocating records is certainly cheaper in memory; however, the benefits of clustering are more subtle.
On the other hand, moving records across the disk is more expensive, but,
	having records physically clustered on disk can have more substantial performance improvements
	in subsequent query executions.
Therefore, using \tunableLSH in a disk-based system is a matter of 
	reconfiguring how frequently physical clustering takes place.
In fact, it is even possible to use multiple \tunableLSH schemes concurrently 
	at different levels of the memory hierarchy, which is part of our future work.

